Generalized Category Discovery

In this paper, we consider a highly general image recognition setting wherein, given a labelled and unlabelled set of images, the task is to categorize all images in the unlabelled set. Here, the unlabelled images may come from labelled classes or from novel ones. Existing recognition methods are not able to deal with this setting, because they make several restrictive assumptions, such as the unlabelled instances only coming from known - or unknown - classes, and the number of unknown classes being known a-priori. We address the more unconstrained setting, naming it 'Generalized Category Discovery', and challenge all these assumptions. We first establish strong baselines by taking state-of-the-art algorithms from novel category discovery and adapting them for this task. Next, we propose the use of vision transformers with contrastive representation learning for this open-world setting. We then introduce a simple yet effective semi-supervised $k$-means method to cluster the unlabelled data into seen and unseen classes automatically, substantially outperforming the baselines. Finally, we also propose a new approach to estimate the number of classes in the unlabelled data. We thoroughly evaluate our approach on public datasets for generic object classification and on fine-grained datasets, leveraging the recent Semantic Shift Benchmark suite. Project page at https://www.robots.ox.ac.uk/~vgg/research/gcd

==> fig/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{fig/overview_fig.pdf}
\end{center}
\caption{Overview of our proposed `Generalized Novel Category Discovery' setting and method. Our setting can be succinctly described as: given a dataset, a subset of which has class labels, categorize all unlabelled images in the dataset. Our method leverages the properties of contrastively trained vision transformers to assign labels directly through clustering.}
\label{fig:overview}
\end{figure*}

==> fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{fig/teaser_fig.pdf}
\end{center}
\caption{We propose `\settingname', a less constrained image recognition task than the related problems of semi-supervised learning, open-set recognition, and novel category discovery.}
\label{fig:teaser}
\end{figure}

==> sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> tab/sota.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
% 
\textbf{State of the art} -- Glory to the bold numbers.
% 
} % \caption
\label{tab:sota}
\end{table}

==> vaze22gcd_orig copy/fig/attention_viz.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.\textwidth]{fig/attention_viz_fig.pdf}
\end{center}
\caption{Attention visualizations for the DINO-ViT model before (left) and after (right) fine-tuning with our approach. For Stanford Cars and CUB, we show an image from the `Old' (first row for each dataset) and `New' classes (second row for each dataset). Our model learns to specialize attention heads (shown as columns) to different semantically meaningful parts, which can transfer between the labelled and unlabelled categories. The model's heads learn `Windshield', `Headlight' and `Wheelhouse' for the cars, and `Beak', `Head' and 'Belly' for the birds. For both models, we select heads with as focused attention as possible. Recommended viewing in color with zoom.}
\label{fig:attention}
\end{figure*}

==> vaze22gcd_orig copy/fig/hugarian_and_acc_diagram.tex <==
\begin{figure*}[t!]
\begin{center}
\includegraphics[width=\textwidth]{fig/hungarian_and_acc_diagram.pdf}
\end{center}
\caption{An illustration of how the Hungarian algorithm affects the final clustering $ACC$. The left-hand image shows two discovered clusters (`Cluster 1' and `Cluster 2') and the ground truth labels of their constituent instances (solid colored circles). On the right, we show how $ACC$ is computed if the Hungarian assignment is computed only once (`Ours') as well as how $ACC$ is computed if the Hungarian assignment is computed independently for `Old' and `New' classes (`Legacy NCD').}
\label{fig:hungarian_and_acc}
\end{figure*}

==> vaze22gcd_orig copy/fig/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{fig/overview_fig.pdf}
\end{center}
\caption{Overview of our proposed `Generalized Novel Category Discovery' setting and method. Our setting can be succinctly described as: given a dataset, a subset of which has class labels, categorize all unlabelled images in the dataset. Our method leverages the properties of contrastively trained vision transformers to assign labels directly through clustering.}
\label{fig:overview}
\end{figure*}

==> vaze22gcd_orig copy/fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{fig/teaser_fig.pdf}
\end{center}
\caption{We propose `\settingname', a less constrained image recognition task than the related problems of semi-supervised learning, open-set recognition, and novel category discovery.}
\label{fig:teaser}
\end{figure}

==> vaze22gcd_orig copy/fig/tsne.tex <==
\begin{figure*}[htb]
\begin{center}
\includegraphics[width=1.\linewidth]{fig/tsne_fig.pdf}
\end{center}
\caption{TSNE visualization of instances in CIFAR10 for features generated by a ResNet-50 and ViT model trained with DINO self-supervision on ImageNet, and a ViT model after fine-tuning with our approach.}
\label{fig:tsne}
\end{figure*}

==> vaze22gcd_orig copy/sec/0_abstract.tex <==
\begin{abstract}
In this paper, we consider a highly general image recognition setting wherein, given a labelled and unlabelled set of images, the task is to categorize all images in the unlabelled set.
Here, the unlabelled images may come from labelled classes or from novel ones.
Existing recognition methods are not able to deal with this setting, because they make several restrictive assumptions, such as the unlabelled instances only coming from known -- or unknown -- classes, and the number of unknown classes being known a-priori. 
We address the more unconstrained setting, naming it `Generalized Category Discovery', and challenge all these assumptions. 
We first establish strong baselines by taking state-of-the-art algorithms from novel category discovery and adapting them for this task.
Next, we propose the use of vision transformers with contrastive representation learning for this open-world setting. 
We then introduce a simple yet effective semi-supervised $k$-means method to cluster the unlabelled data into seen and unseen classes automatically, substantially outperforming the baselines. 
Finally, we also propose a new approach to estimate the number of classes in the unlabelled data. 
We thoroughly evaluate our approach on public datasets for generic object classification and on fine-grained datasets, leveraging the recent Semantic Shift Benchmark suite. Code: \href{https://www.robots.ox.ac.uk/~vgg/research/gcd/}{https://www.robots.ox.ac.uk/$\sim$vgg/research/gcd}
\end{abstract}

==> vaze22gcd_orig copy/sec/0_metadata.tex <==
\title{Generalized Category Discovery}

\author{Sagar Vaze$^\star$ \qquad Kai Han$^\dagger$ \qquad Andrea Vedaldi$^\star$ \qquad Andrew Zisserman$^\star$\\
\small 
$^\star$Visual Geometry Group, Department of Engineering Science, University of Oxford \\
% The Weizmann Institute of Science\\
\small
$^\dagger$The University of Hong Kong\\
{\tt\small \{sagar,vedaldi,az\}@robots.ox.ac.uk \qquad kaihanx@hku.hk}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
}

==> vaze22gcd_orig copy/sec/1_introduction.tex <==
\section{Introduction}\label{sec:intro}

Consider an infant sitting in a car and observing the world.
Object instances will pass the car and, for some of these, the infant may have been told their category (`that is a dog', `that is a car') and be able to recognize them.
There will also be instances that the infant has not seen before (cats and bicycles) and, having seen a number of these instances, we might expect the infant's visual recognition system to cluster these into new categories.

This is the problem that we consider in this work:
given an image dataset where only some images are labelled with their categories, assign a category label to each of the rest images, possibly using new categories not observed in the labelled set.
We term this problem \textit{Generalized Category Discovery} (GCD), and suggest that this is a realistic use case for many machine vision applications: whether that is recognizing products in a supermarket; pathologies in medical images; or vehicles in autonomous driving. 
\todo{In these and other realistic vision settings, it is often impossible to know if new images come from labelled or novel categories.}

In contrast, consider the limitations of existing image recognition settings.
In image classification, one of the most widely studied problems, all of the training images come with class labels.
Furthermore, all images at test time come from the same classes as the training set.
Semi-supervised learning (SSL)~\cite{chapelle2006semi} introduces the problem of learning from unlabelled data, but still assumes that all unlabelled images come from the same set of classes as the labelled ones.
More recently, the tasks of open-set recognition (OSR)~\cite{Scheirer_2013_TPAMI} and novel-category discovery (NCD)~\cite{han2019learning} have tackled open-world settings in which the images at test time may belong to new classes.
However, OSR aims only to \textit{detect} test-time images which do not belong to one of the classes in the labelled set, but does not require any further classification amongst these detected images.
Meanwhile, in NCD, the closest setting to the one tackled in this work, methods learn from labelled and unlabelled images, and aim to discover new classes in the unlabelled set.
However, NCD still makes the limiting assumption that \textit{all} of the unlabelled images come from new categories,  which is usually unrealistic.

In this paper, we tackle Generalized Category Discovery in a number of ways.
Firstly, we establish strong baselines by taking representative methods from NCD and applying them to this task. 
To do this, we adapt their training and inference mechanisms to account for our more general setting, as well as retrain them with a more robust backbone architecture.
We show that existing NCD methods are prone to overfit the labelled classes in this generalized setting. 

Next, observing the potential for NCD methods to overfit their classification heads to the labelled classes, we propose a simple but effective method for recognition by clustering.
Our key insight is to leverage the strong `nearest neighbour' classification property of vision transformers along with contrastive learning.
We propose the use of contrastive training and a semi-supervised $k$-means clustering algorithm to recognize images without a parametric classifier.
We show that these proposed methods substantially outperform the established baselines, both on generic object recognition datasets and, particularly, on more challenging fine-grained benchmarks.
For the latter evaluations, we leverage the recently proposed Semantic Shift Benchmark suite \cite{vaze2022openset}, which was designed for the task of identifying semantic novelty.

Finally, we propose a solution to a challenging and under-investigated problem in image recognition: estimating the number of categories in unlabelled data.
Almost all methods, including purely unsupervised ones, assume the knowledge of the number of categories, a highly unrealistic assumption in the real world.
We propose an algorithm which leverages the labelled set to tackle this problem.

\todo{Our contributions can be summarized as follows:
(i) the formalization of Generalized Category Discovery (GCD), a new and realistic setting for image recognition;
(ii) the establishment of strong baselines by adapting state-of-the-art techniques from standard novel category discovery to this task;
(iii) a simple but effective method for GCD, which uses contrastive representation learning and clustering to directly provide class labels, and outperforms the baselines substantially;
(iv) a novel method for estimating the number of categories in unlabelled data, a largely understudied problem;
and (v) rigorous evaluation on standard image recognition datasets as well as the recent Semantic Shift Benchmark suite \cite{vaze2022openset}. 
}

% \begin{itemize}[leftmargin=*]
% \setlength\itemsep{-.3em}
% \item The formalization of Generalized Category Discovery (GCD), a new setting for image recognition.
% \item The establishment of strong baselines by transferring and adapting state-of-the-art techniques from standard novel category discovery to this task.
% \item A simple but effective method for GCD, which uses contrastive representation learning and clustering to directly provide class labels, and outperforms the baselines substantially.
% \item A novel method for estimating the number of categories in unlabelled data, a largely understudied problem.
% \item \todo{SSB}
% \end{itemize}


% We hope that this paper will serve as a springboard for future work on this more realistic version of open world image recognition.

==> vaze22gcd_orig copy/sec/2_related.tex <==
 %< bloody latex and its heuristics for figure placement

\section{Related work}
\label{sec:related}

Our work relates to prior work on \textit{semi-supervised learning}, \textit{open-set recognition}, and \textit{novel category discovery}, which we briefly review next.

\paragraph{Semi-supervised learning}
A number of methods~\cite{chapelle2006semi,oliver2018realistic,rebuffi2019semi,sohn2020fixmatch,48416} have been proposed to tackle the problem of semi-supervised learning (SSL). 
SSL assumes that the labelled and unlabelled instances come from the same set of classes. 
The objective is to learn a robust classification model leveraging both the labelled and unlabelled data during training. 
Amongst existing methods, consistency based approaches appear to be popular and effective, such as LadderNet~\cite{rasmus2015semi}, PI model~\cite{laine2016temporal}, Mean-teacher~\cite{tarvainen2017mean}. Recently, with the success of self-supervised learning, methods have also been proposed to improve SSL by augmenting the methods with self-supervised objectives~\cite{rebuffi2019semi,48416}. 

\paragraph{Open-set recognition}
The problem of open-set recognition (OSR) is formalized in~\cite{Scheirer_2013_TPAMI}, with the objective being to classify unlabelled instances from the same semantic classes as the labelled data, while detecting test instances from unseen classes. 
OpenMax~\cite{BendaleB15} is the first deep learning method to approach this problem with Extreme Value Theory. GANs are often employed to generate adversarial samples to train an open-set classifier, e.g, \cite{Neal_2018_ECCV,Ge2017Generative,kong2021}. Several methods have been proposed to train models such that images with large reconstruction error are regarded as open-set samples~\cite{Yoshihashi_2019_CVPR,Oza2019C2AE,Sun_2020_CVPR}. There are also methods that learns prototypes for the labelled classes, and identify the images from unknown classes by the distances to the prototypes~\cite{Shu2020podn,Chen_2020_ECCV,chen2021adversarial}.  
More recently, \cite{Chen_2020_ECCV,chen2021adversarial} proposed to learn reciprocal points which describe `otherness' with respect to the labelled classes. 
\cite{openhybrid20} jointly trains a flow-based density estimator and a classification based encoder for OSR. Finally, Vaze et al. \cite{vaze2022openset} study the correlation between the closed-set and open-set performance, showing that state-of-the-art OSR results can be obtained by boosting the closed-set accuracy of the standard cross-entropy baseline.

\paragraph{Novel category discovery}
The problem of novel category discovery (NCD) is formalized in DTC~\cite{han2019learning}. Earlier methods that could be applied to this problem include KCL~\cite{Hsu18_L2C} and MCL~\cite{Hsu19_MCL}, both of which maintain two models trained with labelled data and unlabelled data respectively, for general task transfer learning. 
AutoNovel (aka Rankstats)~\cite{han21autonovel,han20automatically} tackles the NCD problem with a three stage method. 
The model is first trained with self-supervision on all data for low-level representation learning. 
Then, it is further trained with full supervision on labelled data to capture higher level semantic information. Finally, a joint learning stage is carried out to transfer knowledge from the labelled to unlabelled data with ranking statistics.
Zhao and Han~\cite{zhao21novel} propose a model with two branches, one for global feature learning and the other for local feature learning, such that dual ranking statistics and mutual learning are conducted with these two branches for better representation learning and new class discovery.
OpenMix~\cite{zhong2021openmix} mixes the labelled and unlabelled data to avoid the model from over-fitting for NCD. NCL~\cite{Zhong_2021_CVPR} extracts and aggregates the pairwise pseudo-labels for the unlabelled data with contrastive learning and generates hard negatives by mixing the labelled and unlabelled data in the feature space for NCD.
Jia~et al.~\cite{jia21joint} propose an end-to-end NCD method for single- and multi-modal data with contrastive learning and winner-takes-all hashing.
A unified cross-entropy loss is introduced in UNO~\cite{Fini_2021_ICCV} to allow the model to be trained on labelled and unlabelled data jointly, by swapping the pseudo-labels from labelled and unlabelled classification heads.

\todo{Finally, we highlight the work by Girish et al. \cite{girish2020attribution} that tackles a similar setting to GCD but for the task of \textit{GAN attribution} instead of image recognition, as well as the concurrent work by Cao et al. \cite{cao2022openworld} that tackles a similar setting for image recognition under the name \textit{Open World Semi-Supervised Learning}. 
Different to our setting, they do not leverage large-scale pretraining or demonstrate performance on the Semantic Shift Benchmark, which better isolates the problem of detecting semantic novelty.} 

==> vaze22gcd_orig copy/sec/3_method.tex <==
\section{Generalized category discovery}

We first formalize the task of \emph{Generalized Category Discovery} (GCD).
In short, we consider the problem of classifying images in a dataset, a subset of which has known class labels.
The task is to assign class labels to all remaining images, using classes that may or may not be observed in the labelled images (see \cref{fig:overview}, left).

Formally, we define GCD as follows.
We consider a dataset $\mathcal{D}$ comprising two parts
$\mathcal{D_L} = \{(\mathbf{x}_i, y_i)\}_{i=1}^{N} \in \mathcal{X} \times \mathcal{Y_L}$
and
$\mathcal{D_U} = \{(\mathbf{x}_i, y_i)\}_{i=1}^{M} \in \mathcal{X} \times \mathcal{Y_U}$,
where $\mathcal{Y_L} \subset \mathcal{Y_U}$.
During training, the model does not have access to the labels in $\mathcal{D_U}$, and is tasked with predicting them at test time.
Furthermore, we assume access to a validation set,
$\mathcal{D_V} = \{(\mathbf{x}_i, y_i)\}_{i=1}^{N'} \in \mathcal{X} \times \mathcal{Y_L}$,
which is disjoint from the training set and contains images from the same classes as the labelled set.
This formalization allows us to clearly see the distinction with the novel category discovery setting.
NCD assumes $\mathcal{Y_L} \cap \mathcal{Y_U} = \emptyset$ and existing methods rely on this prior knowledge during training.

In this section, we describe the methods we propose to tackle GCD\@.
First, we describe our approach to the problem.
Leveraging recent progress in self-supervised representation learning, we propose a simple but effective approach based on contrastive learning, with classification performed by a semi-supervised $k$-means algorithm.
Next, we develop a method to estimate the number of categories in the unlabelled data -- a challenging task that is understudied in the literature.
Finally, we build two strong baselines for GCD by modifying state-of-the-art NCD methods, RankStats~\cite{han21autonovel} and UNO~\cite{Fini_2021_ICCV}, to fit with our setting.

\subsection{Our approach}

The key insight of our approach for image recognition in an open-world setting is to remove the need for parametric classification heads.
Instead, we perform clustering directly in the feature space of a deep network (see \cref{fig:overview}, right).
Classification heads (typically, linear classifiers on top of a learned embedding) are best trained with the cross-entropy loss, which has been shown to be susceptible to noisy labels~\cite{Lei20can}.
Furthermore, when training a linear classifier for unlabelled classes, a typical method is to generate (noisy) pseudo-labels for the unlabelled instances.
This would suggest that parametric heads are susceptible to performance deterioration on the unlabelled classes.
Finally, we note that, by necessity, classification heads must be trained from scratch, which further makes them vulnerable to overfitting on the labelled classes.

Meanwhile, self-supervised contrastive learning has been widely used as pre-training to achieve robust representations in NCD~\cite{jia21joint,Zhong_2021_CVPR}.
Furthermore, when combined with vision transformers, it generates models which are good nearest neighbour classifiers~\cite{caron2021emerging}.
Inspired by this, we find that constrastively training a ViT model allows us to directly cluster in the model's feature space, thereby removing the need for a linear head which could lead to overfitting.
Specifically, we train the representation with a noise contrastive loss~\cite{gutmann2010noise} on all images \emph{without using any labels}.
This is important because it avoids overfitting the features to the subset of classes that are (partially) labelled.
We add a further supervised contrastive component~\cite{khosla2020supervised} for the labelled instances to make use of the labelled data (see \cref{fig:overview}, middle row on the right).

\subsubsection{Representation learning}

We use, for all methods, a vision transformer (ViT-B-16)~\cite
{dosovitskiy2021an} pretrained with DINO~\cite{caron2021emerging} self-supervision on (unlabelled) ImageNet~\cite{deng09imagnet} as our backbone.
This is motivated firstly because the DINO model is a strong nearest neighbour classifier, which suggests non-parametric clustering in its feature space would work well.
Secondly, self-supervised vision transformers have demonstrated the attractive quality of learning to attend to salient parts of an object without human annotation.
We find this feature to be useful for this task, because \emph{which} object parts are important for classification is likely to transfer well from the labelled to the unlabelled categories (see \cref{sec:qualitative_results}).

Finally, we wish to reflect a realistic and practical setting.
In the NCD literature, it is standard to train a ResNet-18~\cite{he2016deep} backbone from scratch for the target task.
However, in a real-world setting, a model is often initialized with large-scale pretrained weights to optimize performance (often ImageNet supervised pretraining).
In order to avoid conflicts with our experimental setting (which assumes a finite labelled set), we use self-supervised ImageNet weights.
To enhance the representation such that it is more tailored for the labelled and unlabelled data we have, we further fine-tune the representation on our target data jointly with supervised contrastive learning on the labelled data, and unsupervised contrastive learning on \textit{all} the data.

Formally, let $\mathbf{x}_i$ and $\mathbf{x}_{i}'$ be two views (random augmentations) of the same image in a mini-batch $B$.
The unsupervised contrastive loss is written as:
\begin{equation}
\label{eq:nce_unsup}
\mathcal{L}^{u}_{i} =
- \log \frac{\exp \left(\mathbf{z}_i \cdot \mathbf{z}_{i}'/ \tau\right)}{\sum_{n}  \mathds{1}_{[n \ne i]} \exp \left(\mathbf{z}_i \cdot \mathbf{z}_n / \tau\right)},
\end{equation}
where $\mathbf{z}_i = \phi(f(\mathbf{x}_i))$ and $\mathds{1}_{[n \ne i]}$ is an indicator function evaluating to 1 \emph{iff}  $n \ne i$, and $\tau$ is a temperature value. $f$ is the feature backbone, and $\phi$ is a multi-layer perceptron (MLP) projection head.

The supervised contrastive loss is written as:
\begin{equation}
\label{eq:nce_sup}
\medmuskip=2mu
\thickmuskip=3mu
\renewcommand\arraystretch{1.5}
\mathcal{L}^{s}_{i} =
- \frac{1}{|\mathcal{N}(i)|}  \sum_{q \in \mathcal{N}(i)}\log \frac{\exp \left(\mathbf{z}_i \cdot \mathbf{z}_q / \tau\right)}{\sum_{n} \mathds{1}_{[n \ne i]} \exp \left(\mathbf{z}_i \cdot \mathbf{z}_n / \tau\right)},
\end{equation}
where $\mathcal{N}(i)$ denotes the indices of other images having the same label as $\mathbf{x}_i$ in the mini-batch $B$.
Finally, we construct the total loss over the batch as:
\begin{equation}
\label{eq:total_loss}
\mathcal{L}^{t} = (1 - \lambda) \sum_{i \in B} \mathcal{L}^{u}_{i} +
\lambda \sum_{i \in B_\mathcal{L}} \mathcal{L}^{s}_{i}
\end{equation}
where $B_\mathcal{L}$ corresponds to the labelled subset of $B$ and $\lambda$ is a weight coefficient.
Using the labels \textit{only} in a contrastive framework, rather than in a cross-entropy loss, means that unlabelled and labelled data are treated similarly.
The supervised contrastive component is only used to nudge the network towards a semantically meaningful representation, thereby minimizing overfitting on the labelled classes.
% in $\mathcal{Y_L}$.

\subsubsection{Label assignment with semi-supervised $k$-means}
\label{sec:semi_sup_kmeans}

Given the learned representation for the data, we can now assign class or cluster labels for each unlabelled data point, either from the labelled classes or unseen new classes.
Instead of performing this parametrically as is common in NCD (and risk overfitting to the labelled data) we propose to use a non-parametric method.
Namely, we propose to modify the classic $k$-means into a constraint algorithm by forcing the assignment of the instances in $\mathcal{D_L}$ to the correct cluster based on their ground-truth labels. Note, here we assume knowledge of the number of clusters, $k$. We tackle the problem of estimating this parameter 
in \cref{sec:k_estimation}.
The initial $|\mathcal{Y_L}|$ centroids for $\mathcal{D_L}$ are obtained based on the ground-truth class labels, and an additional 
% $u$
$|\mathcal{Y_U}\setminus \mathcal{Y_L}|$
(number of new classes) initial centroids are obtained from $\mathcal{D_U}$ with $k$-means++~\cite{Arthur2008kmeanspp}, constrained on the centroids of $\mathcal{D_L}$.
During each centroid update and cluster assignment cycle, instances from the same class in $\mathcal{D_L}$ are always forced to have the same cluster assignment, while each instance in $\mathcal{D_U}$ can be assigned to any cluster based on the distance to different centroids. After the semi-supervised $k$-means converges, each instance in $\mathcal{D_U}$ can be assigned a cluster label. We provide a clear diagram of this in \cref{sec:semi_sup_kmeans_sup}.

% After training, we make use of a semi-supervised $k$-means algorithm to provide classification labels.
% Specifically, we perform $k$-means clustering over the entire dataset, $\mathcal{D} = \mathcal{D_L} \cup \mathcal{D_U}$.
% On each iteration of the $k$-means algorithm, we force assignment of the instances in $\mathcal{D_L}$ to the correct cluster based on their ground truth labels.
% In this way, the centroid updates for classes in $\mathcal{Y_L}$ are guided by a supervisory signal.

\subsection{Estimating the class number in unlabelled data}
\label{sec:k_estimation}

Here, we tackle the problem of finding the number of classes in the unlabelled data.
In the NCD and unsupervised clustering settings, prior knowledge of the number of categories in the dataset is often assumed, but this is unrealistic in the real world given that the labels themselves are unknown.
To estimate the number of categories in $\mathcal{D_U}$, we leverage the information available in $\mathcal{D_L}$.
Specifically, we perform $k$-means clustering on the entire dataset, $\mathcal{D}$, before evaluating clustering accuracy on \textit{only} the labelled subset (see \cref{evaluation_protocol} for the metric's definition).

Clustering accuracy is evaluated by running the Hungarian algorithm~\cite{kuhn1955hungarian} to find the optimal assignment between the set of cluster indices and ground truth labels.
If the number of clusters is higher than the total number of classes, the extra clusters are assigned to the null set, and all instances assigned to those clusters are said to have been predicted incorrectly.
Conversely, if the number of clusters is lower than the number of classes, extra classes are assigned to the null set, and all instances with those ground truth labels are said to have been to be predicted incorrectly.
Thus, we assume that, if the clustering (across $\mathcal{D}$) is performed with $k$ too high or too low, then this will be reflected in a sub-optimal clustering accuracy on $\mathcal{D_L}$.
In other words, we assume clustering accuracy on the labelled set will be maximized when $k = |\mathcal{Y_L} \cup \mathcal{Y_U}|$.
This intuition leads us to use the clustering accuracy as a `black box' scoring function, $ACC = f(k; \mathcal{D})$, which we optimize with Brent's algorithm to find the optimal $k$.
\todo{Different to the method in \cite{han21autonovel}, which exhaustively iterates through all possible values of $k$, we find that the black-box optimization allows our method to scale to datasets with many categories.

Finally, we highlight that labelled sets with different granularities would induce different estimates of the number of classes. 
However, we suggest that the labelled set defines the system of categorization --- that the granularity of a real-world dataset is not an intrinsic property of the images, but rather a framework imposed by the labels. For instance, in Stanford Cars, the dataset could equally be labelled at the ‘Manufacturer’, ‘Model’ or ‘Variant’ level, with the categorization system defined by the labels assigned.}

\subsection{Two strong baselines}

We adapt two methods from the nearest image recognition sub-field, novel category discovery (NCD), for our generalized category discovery (GCD) task.
\textit{RankStats}~\cite{han21autonovel} is widely used as a competitive baseline for novel category discovery, while \textit{UNO}~\cite{Fini_2021_ICCV} is to the best of our knowledge the state-of-the-art method for NCD\@.

\paragraph{Baseline: RankStats+}
%
RankStats trains two classifiers on top of a shared feature representation:
the first head is fed instances from the labelled set and is trained with the cross-entropy loss, while the second head sees only instances from unlabelled classes (again, in the NCD setting, the labelled and unlabelled classes are disjoint).
% The second head is trained with binary cross-entropy by generating pairwise pseudo-labels for unlabelled images in a batch.
% We refer the reader to~\cite{han21autonovel} for details on pseudo-label generation.
% In our proposed setting, unlabelled instances could belong to any class in the dataset.
% In contrast,
In order to adapt RankStats to GCD, we train it with a single classification head for the total number of classes in the dataset.
We then train the first $|\mathcal{Y_L}|$ elements of the head with the cross-entropy loss, and train the \textit{entire} head with the binary cross-entropy loss with pseudo-labels.

\paragraph{Baseline: UNO+}
%
Similarly to RankStats, UNO is trained with classification heads for labelled and unlabelled data.
The model is then trained in a SwAV-like manner~\cite{caron2020unsupervised}.
First, multiple views (random augmentations) of a batch are generated and fed to the same model.
For the labelled images in the batch, the labelled head is trained with the cross-entropy loss using the ground truth labels.
For the unlabelled images, predictions (logits from the unlabelled head) are gathered for a given view and used as pseudo-labels with which to optimize the loss from \textit{other} views.
To adapt this mechanism, we simply concatenate both the labelled and unlabelled heads, thus allowing generated pseudo-labels for the unlabelled samples to belong to any class in the dataset.

==> vaze22gcd_orig copy/sec/4_results.tex <==
\section{Experiments}

\subsection{Experimental setup}

\paragraph{Data}
%
We demonstrate results on six datasets in our proposed setting.
For each dataset, we take the training set and sample a set of classes for which we have labels during training.
We further sub-sample 50\% of the images from these classes to constitute the labelled set $\mathcal{D_L}$.
The remaining instances from these classes, along with all instances from the other classes, constitute $\mathcal{D_U}$.
We further construct the validation set for the labelled classes from the test or validation split of each dataset.

We first demonstrate results on three generic object recognition datasets: CIFAR10~\cite{Krizhevsky09cifar}, CIFAR100~\cite{Krizhevsky09cifar} and ImageNet-100~\cite{deng09imagnet}.
ImageNet-100 refers to the ImageNet dataset with 100 classes randomly subsampled.
\todo{These datasets establish the methods' performance on well-known datasets in the standard image recognition literature.

We further evaluate on the recently proposed Semantic Shift Benchmark \cite{vaze2022openset} (SSB, including CUB~\cite{cub200} and Stanford Cars~\cite{Cars196}), as well as on Herbarium19~\cite{Chuan19herbarium}.
SSB provides fine-grained evaluation datasets with clear `axes of semantic variation' and further provides categories for $\mathcal{D_U}$ which are delineated from $\mathcal{D_L}$ in a semantically coherent fashion.
Thus, the user can be confident that the recognition system is identifying new classes based on a true semantic signal, rather than simply responding to low-level distributional shifts in the data, as may be the case for generic object recognition datasets.
The long-tailed nature of Herbarium19 adds an additional challenge to the evaluation.
}

% ability to identify categories with abstract class definitions, as may be encountered in settings such as self-driving or animal monitoring in the wild.
% In these cases, the benchmarks clearly define how individual categories differ from
% each other with clear
% In these benchmarks, there are specific `axes of semantic variation' --- e.g., the difference between two bird species in CUB \emph{vs.}~the difference between a dog and a refrigerator in ImageNet.

The fine-grained datasets further reflect many real-world use cases for image recognition systems, which are deployed in constrained environments with many similar objects (\eg products in a supermarket, traffic monitoring, or animal tracking in the wild).
In fact, the Herbarium19 dataset itself represents a real-world use case for GCD: while we are aware of roughly 400k species of plants, and estimate that there are around 80k yet to be discovered, it currently takes roughly 35 years from plant collection to plant species description if performed manually~\cite{Chuan19herbarium}.
We summarize the dataset splits used in our evaluations in~\cref{tab:datasets}, and provide more details in \cref{sec:dataset_details_sup}.

\input{tab/datasets}

\paragraph{Evaluation protocol}\label{evaluation_protocol}
%
For each dataset, we train the models on $\mathcal{D}$ (without access to the ground truth labels in $\mathcal{D_U}$).
At test-time, we measure the clustering accuracy between the ground truth labels $y_i$ and the model's predictions $\hat{y}_i$ as:
\begin{equation}
    ACC = \max_{p \in \mathcal{P(Y_U)}}
    \frac{1}{M}
    \sum_{i=1}^{M}
    \mathds{1}\{y_i = p(\hat{y}_i)\}
\end{equation}
Here, $M = |\mathcal{D_U}|$ and $\mathcal{P(Y_U)}$ is the set of all permutations of the class labels in the unlabelled set.
\todo{Our main metric is $ACC$ on `All' instances, indicating image recognition accuracy across the entire unlabelled set $\mathcal{D_U}$.
We further report values for both the `Old' classes subset (instances in $\mathcal{D_U}$ belonging to classes in $\mathcal{Y_L}$) and `New' classes subset (instances in $\mathcal{D_U}$ belonging to classes in $\mathcal{Y_U} \setminus \mathcal{Y_L}$).

The maximum over the set of permutations is computed via the Hungarian optimal assignment algorithm~\cite{kuhn1955hungarian}.
Importantly, we compute the Hungarian assignment only once, across all categories $\mathcal{Y_U}$, and measure classification accuracy on `Old' and `New' subsets only afterwards.
The interaction between when the Hungarian assignment is performed, and the resultant $ACC$ on the subsets, can be un-intuitive and is elaborated upon in \cref{sec:appendix_eval_metrics_details}.
}


% \subsection{Implementation details}

% \paragraph{Generalized category discovery}
\paragraph{Implementation details}
%
All methods are trained with a ViT-B-16 backbone with DINO pre-trained weights, and use the output \texttt{[CLS]} token as the feature representation.
All methods were trained for 200 epochs, with the best model selected using accuracy on the validation set.
We fine-tune the final transformer block for all methods.

For our method, we fine-tune the final block of the vision transformer with an initial learning rate of 0.1 which we decay with a cosine annealed schedule.
We use a batch size of 128 and $\lambda = 0.35$ in the loss (see \cref{eq:total_loss}).
Furthermore, following standard practise in self-supervised learning, we project the model's output through a non-linear projection head before applying the contrastive loss.
We use the same projection head as in \cite{caron2021emerging} and discard it at test-time.
For the baselines from NCD, we follow the original implementations and learning schedules as far as possible, referring to the original papers for details \cite{han21autonovel,Fini_2021_ICCV}.

% \paragraph{Estimating $k$}
%
Finally, in order to estimate $k$, we run our $k$-estimation method on DINO features extracted from each of the considered benchmarks.
We run Brent's algorithm on a constrained domain for $k$, with the minimum set at $|\mathcal{Y_L}|$ and the maximum set at 1000 classes for all datasets.

\subsection{Comparison with the baselines}

We report results for all compared methods in~\cref{tab:generic} and~\cref{tab:fine_grained}.
As an additional baseline, we also report results when running $k$-means directly on top of raw DINO features (reported as $k$-means).
\todo{~\cref{tab:generic} presents results on the generic object recognition datasets, while ~\cref{tab:fine_grained} shows results on SSB and Herbarium19.
We further show results on the FGVC-Aircraft \cite{maji13fine-grained} evaluation from SSB in \cref{sec:appendix_fgvc_aircraft}.

Overall (across `All' instances in $\mathcal{D_U}$), our method outperforms RankStats+ and UNO+ baselines on the standard image recognition datasets by 9.3\% in absolute terms, and 11.5\% in proportional terms.
Meanwhile, on the more challenging fine-grained evaluations, our method outperforms the baselines by 8.9\% in absolute terms and 27.0\% in proportional terms.

We find that on categories with labelled examples (`Old' classes), the baselines which use parametric classifiers can outperform our method, but this is at the expense of $ACC$ on the `New' categories.
We also found that, if the baselines were trained for longer, they would begin to sacrifice $ACC$ on `Old' categories for $ACC$ on `New' ones, but that best overall performance was achieved using early stopping by monitoring the performance on the validation set.
}

%(see \ref{})

% We note that, on all datasets, the best performance aggregated over the entire unlabelled set is achieved by our method.
% Our model further outperforms the baselines in most subcategories of the datasets.
% The exception is ImageNet-100, where raw DINO features perform better on the `New' classes (with no labels available in $\mathcal{D}$) and UNO+ performs better on the `Old' ones (from the same classes as those in $\mathcal{D_L}$).
% The first result is explained as DINO is trained in a self-supervised manner on the entire ImageNet dataset, where it has been carefully tuned to achieve a strong representation for all classes.
% We suggest that the second result is due to ImageNet-100 containing many classes, but also containing enough images ($\approx$650) per class to reliably train a linear classifier with cross-entropy.
% In this regime, in the supervised setting, it is still difficult to beat a standard classification head.
% Nonetheless, the best tradeoff between the `New' and `Old' classes is still achieved by our approach.
% We also note that the methods based on parametric classifiers show a substantial discrepancy between their performances on the `Old' and `New' classes, demonstrating overfitting on the labelled categories.
% Across `All' classes in \cref{tab:generic}, on average, our method outperforms the nearest baseline by 6.9\% in absolute terms, and by 9.6\% in proportional terms.

% The results on the FGVC datasets are shown in~\cref{tab:fine_grained}.
% In this more challenging setting, our approach outperforms the baselines substantially in all cases except for the `Old' classes in Herbarium19.
% In this case, RankStats+ demonstrates strong performance, though it once again overfits to the `Old' classes and underperforms our method significantly over `All' classes.
% On the FGVC datasets, we find our method outperforms the nearest baseline by 11.6\% on average in absolute terms, and 34.7\% in proportional terms.

\input{tab/generic}
\input{tab/fine_grained}
\input{fig/tsne}
\input{tab/k_est}
\input{tab/ablation}
\input{fig/attention_viz}

\subsection{Estimating the number of classes}

We report results on estimating the number of classes in~\cref{tab:k_est}.
We find that on the generic object recognition datasets, we can come very close to the ground truth number of categories in the unlabelled set, with a maximum error of 10\%.
On the fine-grained datasets, we report an average discrepancy of 18.9\%.
We note the highly challenging nature of these datasets, with many constituent classes which are visually similar.

\subsection{Ablation study}

In~\cref{tab:ablation}, we inspect the contributions of the various elements of our proposed approach.
Specifically, we identify the importance of the following components of the method: ViT backbone; contrastive fine-tuning (regular and supervised); and semi-supervised $k$-means clustering.

\paragraph{ViT Backbone} Rows (1) and (2) show the effect of the ViT model for the clustering task, as (1) and (2) represent a ResNet-50 model and ViT-B-16 trained with DINO respectively.
The ResNet model performs nearly 20\% worse aggregated over `Old' and `New' classes.
To disambiguate this from the general capacity of the architecture, note that the ImageNet linear probe discrepancy (the standard evaluation protocol for self-supervised models) is roughly 3\%~\cite{caron2021emerging}.
Meanwhile, the discrepancy in their $k$-NN accuracies on ImageNet is roughly 9\%~\cite{caron2021emerging}, suggesting why the ViT model performs so much better for the clustering task.

\paragraph{Contrastive fine-tuning} Rows (2)-(5) show the effects of introducing different combinations of contrastive fine-tuning on the target dataset.
We find that including any of the contrastive methods alone gives relatively marginal improvements over using the raw DINO features.
We find that the full benefit is only realized when combining the self-supervised and supervised contrastive losses on the target dataset.
Specifically, the combination of the contrastive losses allows us to boost aggregated clustering accuracy by a further 19\% on CIFAR100 and by 16\% on Herbarium19 (more than doubling the $ACC$ in this case).

% \paragraph{Semi-supervised $k$-means} The semi-supervised clustering also improves $ACC$ across the board.
% In general, we found that semi-supervised clustering was beneficial on all datasets, and gave a particular boost on the FGVC benchmarks.
% For instance, in the Herbarium19 case, it improves aggregated $ACC$ by nearly 10\%.

\todo{\paragraph{Semi-supervised $k$-means} Further performance gains can be realized with semi-supervised clustering.
Across `All' classes, we observe a 2\% and 7\% increase in $ACC$ on CIFAR100 and Herbarium19 respectively.
On Herbarium19, $ACC$ on the `Old' classes is improved by 19\%.
Interestingly, it appears that semi-supervised $k$-means slightly hurts performance on the `Old' classes on CIFAR100. 
We suggest that this is an artefact of the Hungarian algorithm, which opts to assign some `clean' clusters to the `New' ground truth categories, to maximize overall $ACC$.
This can be observed in the 10\% boost provided by the semi-supervised method on the `New' classes in CIFAR100.
Furthermore, we found that if we performed the Hungarian algorithm on `Old' and `New' instances independently (allowing the reuse of clean clusters during evaluation), semi-supervised $k$-means improved $ACC$ on all data subsets.
We refer to \cref{sec:appendix_eval_metrics_details} for more details on the interaction between the reported $ACC$ and the Hungarian assignment.
}

\paragraph{Summary} Overall, we find that none of the components of our method are individually sufficient to achieve good performance across our benchmark datasets.
Specifically, the \textit{combination} of a vision transformer backbone and contrastive fine-tuning facilitates strong $k$-means clustering directly in the feature space of the model.
The semi-supervised $k$-means algorithm further allows us to guide the
clustering process with labels and achieve better $ACC$, especially on the `New' classes in the fine-grained datasets.

We further illustrate this point in the TSNE visualizations in~\cref{fig:tsne}, performed on the CIFAR10 dataset.
We show TSNE projections of raw ResNet-50 and ViT DINO features, as well as those of our model.
For the ResNet-50 features, points from the same class are generally projected close to each other, indicating that they are likely to be separable given a simple transformation (\eg a linear probe).
However, they do not form clear clusters, hinting at these features' poor down-stream clustering performance.
In contrast, the ViT features form far clearer clusters, which are further distinguished when trained with our approach.

\subsection{Qualitative results}\label{sec:qualitative_results}

Finally, we visualize the attention mechanism of our model to better understand its performance.
Specifically, in~\cref{fig:attention} we look at how the final multi-head attention layer attends to different spatial locations when supporting the output \texttt{[CLS]} token (which we use as our feature representation).
We show this both for the pre-trained DINO model and after training with our method.
We visualize the attention maps for images from the `Old' and `New' classes for Stanford Cars and CUB\@.

It is demonstrated in~\cite{caron2021emerging}  that different attention heads in the DINO model focus on different regions of an image, without the need for human annotation.
We find this to be the case, with different heads attending to disjoint regions of the image and typically focusing on important parts.
However, after training with our method, we find heads to be more specialized to semantic parts, displaying more concentrated and local attention.
In this way, we suggest the model learns to attend to a set of parts which are transferable between the `Old' and `New' classes, which allows it to better generalize knowledge from the labelled data.





==> vaze22gcd_orig copy/sec/5_conclusions.tex <==
\section{Conclusion}

% We have proposed and investigated GCD, a more general, challenging and realistic variant of NCD.
% Given a dataset with partial labels for images and classes, the task is to find the assignment for all unlabelled images, while discovering any new classes.
% % We believe this is a highly general setting which realistically reflects a large number of real-world scenarios. 
% We have developed baselines for the task by transferring state-of-the-art algorithms from NCD and further developed a simple but effective algorithm which substantially outperforms these baselines.
% We also proposed a method for identifying the number of categories in the unlabelled data, which is an understudied problem of practical significance. 
% We hope that this work can serve as a foundation from which to tackle this important problem.

In this paper, we have proposed a new setting for image recognition, `Generalized Category Discovery' (GCD).
We highlight three take-home messages from this work:
first, GCD is a challenging and realistic setting for image recognition;
second, GCD removes limiting assumptions in existing image recognition sub-fields such as novel category discovery and open-set recognition; 
and third, while parametric classifiers tend to overfit to labelled classes in the generalized setting, direct clustering of features from contrastively trained ViTs proves to be a surprisingly good method for classification.

\todo{\noindent\paragraph{Acknowledgements} We would like to thank Liliane Momeni for invaluable help with figures in this work.
This research is funded by a Facebook AI Research Scholarship, a Royal Society Research Professorship RP\textbackslash R1\textbackslash 191132, and the
EPSRC Programme Grant VisualAI EP/T028572/1.}



==> vaze22gcd_orig copy/sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> vaze22gcd_orig copy/tab/ablation.tex <==
\begin{table*}[htb]
\footnotesize
\centering
\caption{Ablation study on the different components of our approach.}\label{tab:ablation}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{}         & \multirow{2}{*}{ViT Backbone} & \multirow{2}{*}{Contrastive Loss} & \multirow{2}{*}{Sup. Contrastive Loss} & \multirow{2}{*}{Semi-Sup $k$-means} & \multicolumn{3}{c}{CIFAR100}                                                          & \multicolumn{3}{c}{Herbarium19}                                                       \\ 
\cmidrule(rl){6-8}
\cmidrule(rl){9-11}
% \cmidrule(rl){8-10}
% \cline{6-11} 
                          &                      &                              &                                   &                                     & \multicolumn{1}{c}{All}  & \multicolumn{1}{c}{Old}  & New                            & \multicolumn{1}{c}{All}  & \multicolumn{1}{c}{Old}  & New                            \\ 
\midrule
\multicolumn{1}{c}{(1)} & \xmark                   & \xmark                           & \xmark                                & \xmark                                  & \multicolumn{1}{c}{34.0} & \multicolumn{1}{c}{34.8} & 32.4                           & \multicolumn{1}{c}{12.1} & \multicolumn{1}{c}{12.5} & 11.9                           \\ 
\multicolumn{1}{c}{(2)} & \cmark                  & \xmark                           & \xmark                                & \xmark                                  & \multicolumn{1}{c}{52.0} & \multicolumn{1}{c}{52.2} & 50.8                           & \multicolumn{1}{c}{12.9} & \multicolumn{1}{c}{12.9} & 12.8                           \\ 
\multicolumn{1}{c}{(3)} & \cmark                  & \cmark                          & \xmark                                & \xmark                                  & \multicolumn{1}{c}{54.6} & \multicolumn{1}{c}{54.1} & 53.7                           & \multicolumn{1}{c}{14.3} & \multicolumn{1}{c}{15.1} & 13.9                           \\ 
\multicolumn{1}{c}{(4)} & \cmark                  & \xmark                           & \cmark                               & \xmark                                  & \multicolumn{1}{c}{60.5} & \multicolumn{1}{c}{72.2} & 35.0                           & \multicolumn{1}{c}{17.8} & \multicolumn{1}{c}{22.7} & 15.4                           \\
\multicolumn{1}{c}{(5)} & \cmark                  & \cmark                          & \cmark                               & \xmark                                  & \multicolumn{1}{c}{71.1} & \multicolumn{1}{c}{\textbf{78.3}} & 56.6 & \multicolumn{1}{c}{28.7} & \multicolumn{1}{c}{32.1} & 26.9                          \\
\multicolumn{1}{c}{(6)} & \cmark                  & \cmark                          & \cmark                               & \cmark                                 & \multicolumn{1}{c}{\textbf{73.0}} & \multicolumn{1}{c}{76.2} & \textbf{66.5}                          & \multicolumn{1}{c}{\textbf{35.4}} & \multicolumn{1}{c}{\textbf{51.0}} & \textbf{27.0} \\ 
\bottomrule
\end{tabular}
\end{table*}


% \begin{table*}[htb]
% \footnotesize
% \centering
% \caption{Ablation.}\label{tab:ablation}
% \begin{tabular}{l|l|l|l|l|lll|lll|}
% \cline{2-11}
% \multirow{2}{*}{}         & \multirow{2}{*}{ViT} & \multirow{2}{*}{Contrastive} & \multirow{2}{*}{Sup. Contrastive} & \multirow{2}{*}{Semi-Sup $k$-means} & \multicolumn{3}{l|}{CIFAR100}                                                          & \multicolumn{3}{l|}{Herbarium19}                                                       \\ \cline{6-11} 
%                           &                      &                              &                                   &                                     & \multicolumn{1}{l|}{All}  & \multicolumn{1}{l|}{Old}  & New                            & \multicolumn{1}{l|}{All}  & \multicolumn{1}{l|}{Old}  & New                            \\ \hline
% \multicolumn{1}{|l|}{(1)} & No                   & No                           & No                                & No                                  & \multicolumn{1}{l|}{34.0} & \multicolumn{1}{l|}{34.8} & 32.4                           & \multicolumn{1}{l|}{12.1} & \multicolumn{1}{l|}{12.5} & 11.9                           \\ \hline
% \multicolumn{1}{|l|}{(2)} & Yes                  & No                           & No                                & No                                  & \multicolumn{1}{l|}{52.0} & \multicolumn{1}{l|}{53.7} & 51.1                           & \multicolumn{1}{l|}{14.1} & \multicolumn{1}{l|}{14.7} & 13.3                           \\ \hline
% \multicolumn{1}{|l|}{(3)} & Yes                  & Yes                          & No                                & No                                  & \multicolumn{1}{l|}{54.6} & \multicolumn{1}{l|}{54.1} & 53.7                           & \multicolumn{1}{l|}{14.3} & \multicolumn{1}{l|}{15.1} & 13.9                           \\ \hline
% \multicolumn{1}{|l|}{(4)} & Yes                  & No                           & Yes                               & No                                  & \multicolumn{1}{l|}{60.5} & \multicolumn{1}{l|}{72.2} & 35.0                           & \multicolumn{1}{l|}{17.8} & \multicolumn{1}{l|}{22.7} & 15.4                           \\ \hline
% \multicolumn{1}{|l|}{(5)} & Yes                  & Yes                          & Yes                               & No                                  & \multicolumn{1}{l|}{73.4} & \multicolumn{1}{l|}{80.9} & \textbf{58.5} & \multicolumn{1}{l|}{27.4} & \multicolumn{1}{l|}{28.0} & 26.9                           \\ \hline
% \multicolumn{1}{|l|}{(6)} & Yes                  & Yes                          & Yes                               & Yes                                 & \multicolumn{1}{l|}{\textbf{73.6}} & \multicolumn{1}{l|}{\textbf{82.3}} & 56.4                           & \multicolumn{1}{l|}{\textbf{37.5}} & \multicolumn{1}{l|}{\textbf{39.5}} & \textbf{35.8} \\ \hline
% \end{tabular}
% \end{table*}



==> vaze22gcd_orig copy/tab/datasets.tex <==
\begin{table}
\centering
\caption{
% 
% \textbf{Datasets}.
Datasets used in our experiments. We show the number of classes in the labelled and unlabelled sets ($|\mathcal{Y_L}|, |\mathcal{Y_U}|$), as well as the number of images ($|\mathcal{D_L}|, |\mathcal{D_U}|$).
} % \caption
\label{tab:datasets}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lcccccc}
\toprule
     & CIFAR10 & CIFAR100 & ImageNet-100 & CUB  & SCars & Herb19 \\ 
\midrule
$|\mathcal{Y_L}|$ & 5       & 80       & 50           & 100  & 98    & 341    \\ 
$|\mathcal{Y_U}|$ & 10      & 100      & 100          & 200  & 196   & 683    \\ 
\midrule
$|\mathcal{D_L}|$ & 12.5k   & 20k      & 31.9k        & 1.5k & 2.0k  & 8.9k   \\ 
$|\mathcal{D_U}|$ & 37.5k   & 30k      & 95.3k        & 4.5k & 6.1k  & 25.4k  \\ 
\bottomrule
\end{tabular}
}
\end{table}

==> vaze22gcd_orig copy/tab/fgvc_aircraft.tex <==
\begin{table}[htb]
\footnotesize
\centering
\caption{Results on the FGVC-Aircraft \cite{maji13fine-grained} splits  from the Semantic Shift Benchmark suite \cite{vaze2022openset}.}\label{tab:appendix_fgvc_aircraft}
% \resizebox{0.33\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lccc}
\toprule
& \multicolumn{3}{c}{FGVC-Aircraft} \\
\cmidrule(rl){2-4}
Classes       & All      & Old     & New \\\midrule
$k$-means~\cite{MackQueen67_Kmeans}
& 16.0
& 14.4
& 16.8
\\
RankStats+
& 26.9
& 36.4
& 22.2
\\
UNO+ 
& 40.3
& \textbf{56.4}
& 32.2
\\
\midrule
Ours
& \textbf{45.0}
& 41.1
& \textbf{46.9}
\\
\bottomrule
\end{tabular}
% }
\end{table}

==> vaze22gcd_orig copy/tab/fine_grained.tex <==
\begin{table}[htb]
\footnotesize
\centering
\caption{Results on SSB \cite{vaze2022openset} and Herbarium19\cite{Chuan19herbarium}. }\label{tab:fine_grained}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lccccccccc}
\toprule
& \multicolumn{3}{c}{CUB} & \multicolumn{3}{c}{Stanford Cars} & \multicolumn{3}{c}{Herbarium19}\\
\cmidrule(rl){2-4}
\cmidrule(rl){5-7}
\cmidrule(rl){8-10}
Classes       & All      & Old     & New        & All       & Old       & New       & All       & Old       & New \\\midrule
$k$-means~\cite{MackQueen67_Kmeans}
& 34.3
& 38.9
& 32.1
& 12.8
& 10.6
& 13.8
& 12.9
& 12.9
& 12.8
\\
RankStats+
& 33.3
& 51.6
& 24.2
& 28.3
& 61.8
& 12.1
& 27.9
& \textbf{55.8}
& 12.8
\\
UNO+ 
& 35.1
& 49.0
& 28.1
& 35.5
& \textbf{70.5}
& 18.6
& 28.3
& 53.7
& 14.7
\\
\midrule
Ours
& \textbf{51.3}
& \textbf{56.6}
& \textbf{48.7}
& \textbf{39.0}
& 57.6
& \textbf{29.9}
& \textbf{35.4}
& 51.0
& \textbf{27.0}
\\
\bottomrule
\end{tabular}
}
\end{table}

==> vaze22gcd_orig copy/tab/generic.tex <==
% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
% \toprule
% Method & Frobnability & Frobnability & Frobnability \\
% \midrule
% Ours v0 & Frumpy \\
% Ours v1 & Frobbly \\
% \textbf{Ours} & Makes one's heart Frob\\
% \bottomrule
% \end{tabular}
% } %< \resizebox
% \caption{
% % 
% \textbf{Ablations} -- our decisions are well justified.
% % 
% } % \caption
% \label{tab:ablations}
% \end{table}



\begin{table}[htb]
\footnotesize
\centering
\caption{Results on generic image recognition datasets.}\label{tab:generic}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lccccccccc}
\toprule
& \multicolumn{3}{c}{CIFAR10} & \multicolumn{3}{c}{CIFAR100} & \multicolumn{3}{c}{ImageNet-100
}\\
\cmidrule(rl){2-4}
\cmidrule(rl){5-7}
\cmidrule(rl){8-10}
Classes       & All      & Old     & New        & All       & Old       & New       & All       & Old       & New \\\midrule
%\\
$k$-means~\cite{MackQueen67_Kmeans}
& 83.6
& 85.7
& 82.5
& 52.0
& 52.2
& 50.8
& 72.7
& 75.5
& \textbf{71.3}
\\
RankStats+
&  46.8
&  19.2
&  60.5
&  58.2
&  77.6
&  19.3
&  37.1
&  61.6
&  24.8
\\
UNO+ 
&  68.6
&  \textbf{98.3}
&  53.8
&  69.5
&  \textbf{80.6}
&  47.2
&  70.3
&  \textbf{95.0}
&  57.9
\\
\midrule
Ours
&  \textbf{91.5}
&  97.9
&  \textbf{88.2}
&  \textbf{73.0}
&  76.2
&  \textbf{66.5}
&  \textbf{74.1}
&  89.8
&  66.3
\\
\bottomrule
\end{tabular}
}
\end{table}

==> vaze22gcd_orig copy/tab/k_est.tex <==
\begin{table}
\centering
\caption{
% 
% \textbf{Finding K}.
Estimation of the number of classes in unlabelled data.
% 
} % \caption
\label{tab:k_est}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lcccccc@{}}
\toprule
   &CIFAR10 &CIFAR100 &ImageNet-100 & CUB & SCars & Herb19 \\
\midrule
Ground truth  
&10
&100
&100
&200
&196
&683
\\
Ours
&9
&100
&109
&231
&230
&520
\\
Error
&10\%
&0\%
&9\%
&16\%
&15\%
&28\%
\\
\bottomrule
\end{tabular}
} % \resizebox

\end{table}

==> vaze22gcd_orig copy/tab/sota.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
% 
\textbf{State of the art} -- Glory to the bold numbers.
% 
} % \caption
\label{tab:sota}
\end{table}
